CarnegiePLUG: Prosumer-in-the-Loop simUlation Grid

This paper introduces Carnegie Mellon campus-wide CarnegiePLUG test-bed. This test-bed in a hardware-in-the-loop simulator that enables large-scale sensing, computation and actuation over a network of heterogeneous energy producers and consumers (prosuming) assets. CarnegiePLUG is a multi-agent framework that facilitates plug-and-play integration of a wide range of virtual and physical sensors and controllers through a multi-layer architecture. Virtual functionalities are accessed in software environments that interface with communication layer of our test-bed. This paper discusses CarnegiePLUG layers, provides implementation details and showcases potential applications of this test-bed through preliminary results.

==> Carolyn-References.tex <==
[1]C. D. Corbin, D. Vrabie, and S. Katipamula, “Co-Simulation and Validation of Advanced Building Controls with $\textpm{VOLTTRON}^{\textpm{TM}}$ and $\textpm{EnergyPlus}^{\textpm{TM}}$,” p. 3-5, 2017.
[2]“External Interface(s) Application Guide,” $\textpm{EnergyPlus}^{\textpm{TM}}$ Version 9.2.0 Documentation, U.S. Department of Energy, p. 5-14, September 27, 2019.
[3]“Getting Started,” $\textpm{EnergyPlus}^{\textpm{TM}}$ Version 9.2.0 Documentation, U.S. Department of Energy, p. 34-35, September 27, 2019.
[4]M. A. Praprost, “Investigating $\textpm{EnergyPlus}^{\textpm{TM}}$ as a Simulation Tool for Deploying $\textpm{VOLTTRON}^{\textpm{TM}}$ Transactive Energy Technologies in Commercial Buildings,” p. 22, 49-63, Case Western Reserve University, 2018.
[5]S. Huang, W. Wang, M. R. Brambley, S. Goyal, and W. Zuo, “An agent-based hardware-in-the-loop simulation framework for building controls,” Energy and Buildings, vol. 181, pp. 12–21, 2018.
[6]Michael Wetter, Wangda Zuo, Thierry S. Nouidui and Xiufeng Pang.
Modelica Buildings library. Journal of Building Performance Simulation, 7(4), 253–270, 2014. DOI:10.1080/19401493.2013.765506 **
[7]J. Haack, B. Akyol, N. Tenney, B. Carpenter, and R. Pratt, “VOLTTRON: An agent platform for the Smart Grid,” Proceedings of the 12th International Conference on Autonomous Agents and Multiagent Systems (AAMAS 2013), 2013.



==> Preliminary-Collaborative.tex <==

Collaborative work together make us ... 
